Towards Edge General Intelligence via Large Language Models: Opportunities and Challenges

Edge Intelligence (EI) has been instrumental in delivering real-time, localized services by leveraging the computational capabilities of edge networks. The integration of Large Language Models (LLMs) empowers EI to evolve into the next stage: Edge General Intelligence (EGI), enabling more adaptive and versatile applications that require advanced understanding and reasoning capabilities. However, systematic exploration in this area remains insufficient. This survey delineates the distinctions between EGI and traditional EI, categorizing LLM-empowered EGI into three conceptual systems: centralized, hybrid, and decentralized. For each system, we detail the framework designs and review existing implementations. Furthermore, we evaluate the performance and throughput of various Small Language Models (SLMs) that are more suitable for development on edge devices. This survey provides researchers with a comprehensive vision of EGI, offering insights into its vast potential and establishing a foundation for future advancements in this rapidly evolving field.

==> Tex/BIO.tex <==
%\begin{IEEEbiographynophoto}{Handi Chen} received the M.Sc. degrees in Network Engineering in 2022 from the Dalian University of Technology, Dalian, China. She is currently working toward the Ph.D. degree in Department of Electrical and Electronic Engineering, the University of Hong Kong, Hong Kong, China. Her research interests include wireless communication, mobile edge computing and privacy preservation.

%\end{IEEEbiographynophoto}

%\begin{IEEEbiographynophoto}{Zhihan Jiang} received the B.E. and M.E. degrees in computer science and technology from Xiamen University, Xiamen, China, in 2018 and 2021, respectively. She is currently pursuing the Ph.D. degree with the Department of Electrical and Electronic Engineering, the University of Hong Kong. Her research interests include Data Analytics and Visualization, Human-Computer Interaction, Ubiquitous Computing, and Mobile Computing.
%\end{IEEEbiographynophoto}
